Peak Value-at-Risk Estimation of Stochastic Processes using Occupation Measures

This paper formulates algorithms to upper-bound the maximum Value-at-Risk (VaR) of a state function along trajectories of stochastic processes. The VaR is upper bounded by two methods: minimax tail-bounds (Cantelli/Vysochanskij-Petunin) and Expected Shortfall/Conditional Value-at-Risk (ES). Tail-bounds lead to a infinite-dimensional Second Order Cone Program (SOCP) in occupation measures, while the ES approach creates a Linear Program (LP) in occupation measures. Under compactness and regularity conditions, there is no relaxation gap between the infinite-dimensional convex programs and their nonconvex optimal-stopping stochastic problems. Upper-bounds on the SOCP and LP are obtained by a sequence of semidefinite programs through the moment-Sum-of-Squares hierarchy. The VaR-upper-bounds are demonstrated on example continuous-time and discrete-time polynomial stochastic processes.

==> sections/acknowledgements.tex <==
\section{Acknowledgements}

\urg{Optional acknowledgements.}
% The authors thank Milan Korda for his discussions about occupation measures and time-varying uncertainty.

==> sections/conclusion.tex <==
\section{Conclusion}

\label{sec:conclusion}

This paper considered the chance-peak problem, which involved finding upper bounds on the quantiles of state functions $p(x)$ achieved by \ac{SDE} systems. The true $(1-\epsilon)$-quantile statistic $P^*$ \eqref{eq:peak_chance} is upper-bounded by the Cantelli/VP approximation $P^*_r$ \eqref{eq:peak_chance_tail}, which in turn is upper bounded by an infinite-dimensional \ac{SOCP} $p^*_r$ \eqref{eq:var_meas_soc} and its moment-\ac{SOS} finite-dimensional \acp{SDP} yielding $p^*_{r,d}$ with $\lim_{d\rightarrow \infty} p^*_{r, d} = p^*_d$. Each of these upper-bounds contribute valuable information towards the analysis of \acp{SDE}.



% \urg{Conclude the paper. Summarize the problem and important findings. Add some extensions and future work.}

% An extended Arxiv version of this paper is available at \urg{[Arxiv link goes here] what will the arxiv version have that this work does not?}.


==> sections/duality_finite.tex <==
\section{Duality and Finite-Dimensional Programs}
\label{sec:duality}
% Compact restriction.

Statement of dual program in terms of an auxiliary function $v(t, x)$

\urg{Possibly put Finite-Dimensional on its own, or lump everything together. I'm not sure how the sectional breakdown will occur. We also have a choice of when to introduce concepts from the Moment-SOS hierarchy. }

% Presentation of Strong duality under the compact setting.

Moment-SOS program with strong duality.



% \urg{ We can't assume that $\mu_p^*$ at optimality will be a dirac delta.}

==> sections/future_work.tex <==
Future work includes finding conditions under which the measure-based upper-bounding does not add conservatism (e.g. cases where $p^*_r = P^*_r$), and utilizing higher-moment tail-probability inequalities to obtain closer estimates to the \ac{VAR} \cite{he2010bounding}. Other work involves studying the duality structure of \eqref{eq:var_meas_soc} with respect to the achievement of strong duality. The techniques introduced in this paper can also be extended to application domains such as distance estimation \cite{miller2022distance_short}, 
\levy processes \cite{kashima2010optimization}, and exit-time statistics \cite{henrion2021moment}. Another avenue involves developing stochastic optimal control strategies to minimize quantile statistics.

==> sections/lmi_converge_note.tex <==
\begin{thm}
\label{thm:lmi_converge}
Under A1-A6, the optima in \eqref{eq:chance_lmi} will converge to \eqref{eq:var_meas_soc} as  $\lim_{d \rightarrow \infty} p^*_{r, d} = p^*_r$.
\end{thm}
\begin{proof}
This convergence will occur by Corollary 8 of \cite{tacchi2022convergence} (when extending to the finite-dimensional \ac{SOC} case) through Lemma \ref{lem:moment_bound}.
\end{proof}

\begin{rmk}
The relation $p^*_d \geq p^*_r \geq P^*_r$ will still hold when $[0, T] \times X$ is noncompact (violating A1 and A5), but it may no longer occur that $\lim_{d \rightarrow \infty} p^*_{r, d} = p^*_r$ (the conditions Lemma \ref{thm:lmi_converge} will no longer apply).
\end{rmk}

==> sections/summary.tex <==

This paper has the following structure: 
Section \ref{sec:preliminaries} gives an overview of notation, \acp{SDE}, and occupation measures. Section \ref{sec:meas} upper-bounds the chance-peak problem using an  infinite-dimensional \ac{SOCP} in  occupation measures.
% Section \ref{sec:duality} provides a dual perspective on this \ac{SOCP} utilizing auxiliary functions \urg{if room allows}. 
Section \ref{sec:lmi} reviews the moment-\ac{SOS} hierarchy and presents a hierarchy of \acp{SDP} that approximate the infinte-dimensional chance-peak \ac{SOCP}. Section \ref{sec:examples} provides numerical examples of the chance-peak problem on \ac{ODE} and \ac{SDE} systems. Section \ref{sec:conclusion} concludes the paper.
% \urg{Fill in the paper structure}
% Section \ref{sec:preliminaries} will review preliminaries such as notation, notions of stability for linear systems, and \ac{SOS} proofs of polynomial nonnegativity. Section \ref{sec:full_method} will present 
% The paper is concluded in Section \ref{sec:conclusion}.

==> sections_arxiv/contributions_arxiv.tex <==
This paper puts forth the following contributions:
\begin{itemize}
    \item Infinite-dimensional convex programs (Minimax \ac{SOCP} and \ac{CVAR} \ac{LP}) to upper-bound the \ac{VAR} of a stochastic process
    \item Converging sequences of \acp{SDP} in increasing size (degree) that upper-bound the infinite-dimensional program using the moment-\ac{SOS} hierarchy
    \item Experiments that demonstrate the utility of these methods on polynomial stochastic systems
    \item Proofs of strong duality and of no-relaxation-gap (between measure programs and \ac{SDE} truth)
\end{itemize}

==> sections_arxiv/future_work_arxiv.tex <==
\old{Future work includes finding conditions under which the measure-based upper-bounding does not add conservatism (e.g., cases where $p^*_r = P^*_r$), and utilizing higher-moment tail-probability inequalities to obtain closer estimates to the \ac{VAR} \cite{he2010bounding}. Another avenue involves developing stochastic optimal control strategies to minimize quantile statistics. Other aspects could include extension of Switching methods towards more general \levy processes \cite{applebaum2004levy, kashima2010optimization}.}

==> sections_tac/biography.tex <==
% \vspace{-0.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/jared_kdd_small.jpg}}]{Jared Miller}  is currently a Post-Doctoral Researcher at the Automatic Control Laboratory (IfA) at ETH Z\"{u}rich, in the research group of Prof. Roy Smith. He received his B.S. and M.S. degrees in Electrical Engineering from Northeastern University in 2018, and his Ph.D. degree from Northeastern University in 2023 under the advisorship of Mario Sznaier (Robust Systems Laboratory). He is a recipient of the 2020 Chateaubriand Fellowship from the Office for Science Technology of the Embassy of France in the United States. He was given an Outstanding Student Paper award at the IEEE Conference on Decision and Control in 2021 and in 2022. His research interests include large-scale convex optimization, semi-algebraic geometry, measure theory, and analysis of nonlinear systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/tacchi}}]{Matteo Tacchi} received a Master's degree in Mathematics from Paris VI University in 2016, and a Ph.D. degree in control theory from Toulouse University in 2021. During his Ph.D., he addressed large scale set approximation problems through convex optimization methods, with application to approximating stability regions of dynamical systems. From 2021 to 2023, he was a postdoctoral fellow with the Automatic Control Laboratory, École Polytechnique Fédérale de Lausanne, working on model and data based optimization for control. He is currently a junior researcher in CNRS GIPSA-lab.
\end{IEEEbiography}

% \vspace{-0.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/Mario18.png}}]{Mario Sznaier}  is currently the Dennis Picard Chaired Professor at the
Electrical and Computer Engineering Department, Northeastern University,
Boston. Prior to joining Northeastern University, Dr. Sznaier
was a Professor of Electrical Engineering at the Pennsylvania State
University and also held visiting positions at the California Institute
of Technology. 
His research interest include robust identification and
control of hybrid systems, robust optimization, and dynamical vision.
Dr. Sznaier is currently serving as Editor in Chief of the section on AI and Control of the journal Frontiers in Control Engineering, and chair of IFAC’s Technical Committee TC 2.5.
Additional  service
includes  Associate Editor for the Journal Automatica (2005-2021),  chair of the CSS Technical Committee on Computational
Aspects of Control System Design (2012-2016), General co-Chair of the 2016 MSC, and Program Chair of the 2017 CDC.
He is a
distinguished member of the IEEE Control Systems Society and an IEEE Fellow.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/Ashkan.max-1000x500.jpg}}]{Ashkan Jasour}  is a Robotics Technologist at NASA’s Jet Propulsion Laboratory (JPL), California Institute of Technology. Before joining JPL, he was a research scientist at the Massachusetts Institute of Technology (MIT). His research focuses on risk-aware planning, control, and optimization under uncertainty for robotic and autonomous systems, with an emphasis on non-Gaussian nonlinear problems. In 2016, he received his PhD in Control Systems/Electrical Engineering and PhD minor in Mathematics from the Pennsylvania State University. He was also a Postdoctoral Associate at MIT’s Computer Science and Artificial Intelligence Laboratory (CSAIL).
\end{IEEEbiography}

==> sections_tac/contributions_above.tex <==
Sections of this research were  presented at the 62nd IEEE Conference on Decision and Control (CDC) \cite{miller2023chancepeak_short}. Contributions in this journal paper above the conference version include:
\begin{itemize}
    \item Non-\ac{SDE} stochastic processes
    \item \ac{CVAR} bounds and \acp{LP}    
    \item Safety analysis through distance estimation
    \item Proofs of no-relaxation-gap and strong duality
\end{itemize}

==> sections_tac/maximin.tex <==
\subsection{Maximin Optimization}

The \ac{CVAR}-maximin problem involves a set of $N_p$ objectives $p_k \in C(X)$ for $k \in 1..N_p$. \ac{CVAR}-maximin replaces the objective of \eqref{eq:peak_cvar_obj} with
\begin{align}
        P^* = & \sup_{t^* \in [0, T] }  \min_{k\in 1..N_p} CVaR_{\epsilon}((p_k)_\# \mu_{t^*}).
\end{align}

Using the maximin framework of Section IV \cite{miller2020recovery} for \acp{ODE}, we supremize a new variable $q \in \R$ such that $q$ lower bounds all of the individual \acp{CVAR} terms $CVaR_{\epsilon}((p_k)_\# \mu_{t^*})$. Variables $(\psi_k, \hat{\psi}_k) \in \Mp{\R}$ are created for each \ac{CVAR} term according to \eqref{eq:cvar_dom}. The resultant maximin \ac{CVAR} program (based on \cite[Equation (20)]{miller2020recovery})  is
\begin{subequations}
\label{eq:peak_cvar_maximin_meas}
\begin{align}
p^* = & \ \sup_{q \in \R} \quad q \label{eq:peak_cvar_maximin_meas_obj} \\
    & \mu_\tau = \delta_0 \otimes\mu_0 + \textstyle \Lie^\dagger \mu \label{eq:peak_cvar_maximin_meas_flow}\\
    & q \leq \inp{\omega}{\psi_k} &  & \forall k\in 1..N_p \\
    & \inp{1}{\psi_k} = 1 & & \forall k\in 1..N_p \label{eq:peak_cvar_maximin_meas_prob}\\
    & \epsilon \psi_k + \hat{\psi_k} = (p_k)_\# \mu_\tau  & & \forall k\in 1..N_p\label{eq:peak_cvar_maximin_meas_cvar}\\
    & \mu_\tau, \ \mu \in \Mp{[0, T] \times X} \label{eq:peak_cvar_maximin_meas_peak}\\    
    & \psi_k, \hat{\psi}_k \in \Mp{\R} & & \forall k\in 1..N_p.\label{eq:peak_cvar_maximin_meas_slack}
\end{align}
\end{subequations}


% \urg{An SDE has independent, stationary increments and also has continuous paths. L\'{e}vy processes remove the requirement that sample paths need to be continuous. The resultant paths can jump a finite number of times in a finite range according to a Poisson point process, assuming that the distribution of the jump heights satisfy a boundedness constraint (L\'{e}vy measure). More information about L\'{e}vy processes are available at \cite{applebaum2004levy}.

% The work in \cite{kashima2010optimization} implemented peak-expectation estimation for \levy processes using (tempered) polynomial optimization. We can use Cantelli/VP bounds to do chance-peak on \levy processes.

% The tempering involved using exponential weights of the 1d state variable when defining all measures, and approximating an exponential*polynomial functions from below by polynomials using a discretezation scheme. It will be exceedingly difficult to generalize the tempering scheme to multiple dimensions due to the curse of dimensionality.

% Depending on time constraints, I might just do arbitrary switching between subsystems and leave it at that.

% } 
